Spatial and dynamical structure of the NGC 2264 star-forming region

The processes that lead from molecular clouds to protostars, stellar associations, and the evolution of both, are active research topics. The target of this study, NGC2264, is a benchmark star-forming region (SFR) in which these issues can be profitably studied. We assembled a new extensive sample of NGC 2264 members. To this end we used new X-ray data obtained with the XMM-Newton telescope, GAIA eDR3 data, and an extensive collection of public and published catalogs. Following a previous suggestion that the SFR might extend significantly beyond the better studied areas, our search covers a wide 2.5x2.5 degrees region in the sky. Our catalog comprises more than 2200 candidate members, a ~100% increase over previous determinations. We analyze their spatial distribution and define new substructures. Using GAIA parallaxes we estimate a new average distance to NGC2264 of 722+/-2pc and suggest that the embedded Spokes subregion is ~20pc farther away within the molecular cloud. A complex dynamics is unveiled by the available proper motions and radial velocities: we observe signs of global expansion and rotation. At the same time, we observe the collapse and coalescence of two substructures in a region where active star formation is taking place. The fraction of stars with disks and of those undergoing circumstellar accretion varies significantly across the field, suggesting that star formation has been occurring for several million years. A particularly low disk fraction around the O VII star S Mon might be attributed to external disk photoevaporation or to an older age of the stars in the region. NGC2264 is not dynamically relaxed and its present configuration is the result of multiple dynamical processes. The cloud has been forming stars for several million years and we identify the process that is likely responsible for the ongoing formation activity.

==> acis12_tab.tex <==
                   n&                R.A.&                Dec.&       $\delta$ pos.\tablefootmark{a}&                Cnts\tablefootmark{b}\\
                    &             [J2000]&             [J2000]&            [arcsec]&                    \\
\hline
         1& 06:40:09.47& +09:53:37.2&       1.2&      13.2\\
         2& 06:40:13.47& +09:53:10.3&       0.9&      15.7\\
         3& 06:40:16.94& +09:46:33.2&       1.0&      14.1\\
         4& 06:40:17.98& +09:50:22.0&       0.8&      11.1\\
         5& 06:40:18.28& +09:44:15.7&       0.9&      18.1\\
         6& 06:40:18.43& +09:52:06.2&       0.6&      20.3\\
         7& 06:40:19.27& +09:48:29.8&       0.3&     120.1\\
         8& 06:40:19.75& +09:31:48.8&       0.6&      62.8\\
         9& 06:40:20.09& +09:56:06.9&       0.9&      12.2\\
        10& 06:40:20.11& +09:45:10.9&       0.3&     165.1\\


==> members_tab.tex <==
             \#&             RA&            Dec&               Gaia Id&                PS1 Id&              2MASS Id&       Mon&      ACIS&       XMM&                                  memb\tablefootmark{a}&                                      field\tablefootmark{b}&                                       samp\tablefootmark{c}\\
               &        [J2000]&        [J2000]&                      &                      &                      &          &          &          &                         &                              &\\
\hline
           4000&    06:40:16.98&    +08:49:27.2&   3326511995354779520&    118581000707459554&      06401697+0849272&     82569&         -&         -&     \verb|0----0---20--|&  \verb|0---1--000-------0100|&\\
           4001&    06:40:16.98&    +10:05:22.8&   3326935066812597248&    120101000707758073&                     -&         -&         -&         -&     \verb|00---0---10--|&  \verb|00--11-000-------0101|&\\
           4002&    06:40:17.00&    +09:46:33.2&   3326714782234731520&    119731000708391565&      06401700+0946332&      1254&         3&         -&     \verb|0000000022101|&  \verb|000000000000--0000000|&bcw\\
           4003&    06:40:17.05&    +09:38:36.6&   3326707124307951232&    119571000710412763&      06401704+0938371&      5872&         -&         -&     \verb|0-0-000020000|&  \verb|0-0000000000--0001110|&\\
           4004&    06:40:17.08&    +09:39:22.3&   3326707154376931840&    119581000711757925&      06401706+0939220&      1169&         -&         -&     \verb|-00------1000|&  \verb|-00-000---0------0000|&cw\\
           4005&    06:40:17.10&    +10:13:35.9&   3326950082019008128&                     -&                     -&      1676&         -&         -&     \verb|-0-------20-0|&  \verb|-0---0-----------00--|&bcw\\
           4006&    06:40:17.10&    +09:39:25.4&   3326707154372788480&    119581000712968943&      06401711+0939254&      5898&         -&         -&     \verb|-00---00-2000|&  \verb|-00-000---00--00-0000|&bcw\\
           4007&    06:40:17.15&    +10:14:37.0&   3326950459975322240&    120291000714492879&      06401715+1014370&      7621&         -&         -&     \verb|-----0-0002--|&  \verb|----000000-----001010|&\\
           4008&    06:40:17.24&    +10:13:35.2&   3326950082018205696&    120271000718382210&      06401724+1013352&      1594&         -&         -&     \verb|0---10--122-0|&  \verb|0--0000000------00000|&bcw\\
           4009&    06:40:17.27&    +09:25:44.2&   3326687917214219008&    119311000719935216&      06401727+0925442&      1261&         -&       350&     \verb|0000000022001|&  \verb|000000000000--0000000|&bcw\\


==> subregions_med.tex <==
\hline
N$_{MMB}$&2257&463&1794&377&1417&387&406&219&80&107&624&175&205&150&55&244\\
N$_{MMB}$(G<17)&821&194&627&143&484&133&172&75&40&57&179&63&68&61&7&48\\
N$_{MMB}$(G<19)&1520&326&1194&282&912&276&313&157&61&95&323&113&118&105&13&92\\
Density [pc$^{-2}$]&0.10&0.02&0.51&0.17&1.10&0.49&1.60&1.11&2.83&3.78&2.45&1.15&4.01&3.32&9.34&4.78\\
X(G<19) - N&827&34&793&127&666&152&214&91&48&75&300&103&109&98&11&88\\
X(G<19) - sel.f&0.64&0.44&0.65&0.48&0.69&0.51&0.65&0.54&0.75&0.77&0.87&0.81&0.88&0.89&0.85&0.92\\
X(G<19) - rej.f&0.13&0.50&0.11&0.32&0.07&0.10&0.05&0.08&0.04&0.03&0.07&0.12&0.05&0.05&0.00&0.03\\
X(G<17) - N&550&22&528&93&435&107&152&65&35&52&176&61&68&62&6&47\\
X(G<17) - sel.f&0.82&0.50&0.83&0.70&0.85&0.75&0.85&0.81&0.85&0.89&0.92&0.87&0.96&0.97&0.86&0.94\\
X(G<17) - rej.f&0.12&0.55&0.11&0.31&0.06&0.09&0.04&0.06&0.03&0.02&0.06&0.10&0.04&0.05&0.00&0.04\\
CoRoT - N&165&44&121&62&59&18&20&12&4&4&21&7&7&6&1&7\\
CoRoT - sel.f&0.69&0.52&0.72&0.72&0.72&0.68&0.66&0.80&0.38&0.67&0.84&0.78&0.78&0.75&1.00&1.00\\
CoRoT - rej.f&0.38&0.75&0.25&0.42&0.07&0.17&0.05&0.00&0.25&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
f$_{mIR}$&0.81&0.85&0.80&0.86&0.79&0.85&0.77&0.80&0.66&0.80&0.76&0.77&0.74&0.85&0.45&0.77\\
f$_{mIR-ex}$&0.45&0.44&0.46&0.33&0.49&0.37&0.41&0.46&0.49&0.27&0.63&0.35&0.66&0.62&0.88&0.80\\
$\sigma$f$_{mIR-ex}$&0.02&0.03&0.02&0.03&0.02&0.03&0.04&0.05&0.10&0.06&0.04&0.05&0.07&0.07&0.19&0.07\\
f$_{H\alpha}$&0.65&0.40&0.72&0.66&0.74&0.81&0.84&0.81&0.89&0.86&0.63&0.78&0.67&0.76&0.42&0.48\\
f$_{acc}$&0.35&0.15&0.37&0.20&0.41&0.28&0.42&0.38&0.58&0.38&0.51&0.35&0.62&0.60&0.74&0.57\\
$\sigma$f$_{acc}$&0.02&0.03&0.02&0.03&0.02&0.03&0.04&0.05&0.09&0.06&0.04&0.05&0.07&0.07&0.18&0.07\\
f$_{dist}$&0.75&0.76&0.75&0.80&0.73&0.82&0.87&0.83&0.86&0.94&0.59&0.75&0.61&0.72&0.33&0.45\\
med(dist)[pc]&726&741&724&715&725&722&725&725&724&725&729&725&728&728&737&741\\
$\sigma$med(dist)[pc]&7&10&8&11&10&13&18&17&57&39&18&25&22&24&58&50\\
f$_{dist.no.out.}$&0.62&0.61&0.63&0.68&0.61&0.72&0.73&0.67&0.73&0.84&0.48&0.65&0.50&0.59&0.25&0.33\\
med(dist.no.out.)[pc]&722&727&722&714&723&721&722&721&722&719&727&724&721&721&723&741\\
$\sigma$med(dist.no.out.)[pc]&2&6&2&5&3&5&4&6&9&9&5&8&7&8&25&9\\
f$_{P.M.}$&0.75&0.76&0.75&0.80&0.73&0.82&0.87&0.83&0.86&0.94&0.59&0.75&0.61&0.72&0.33&0.45\\
med(P.M.$_{R.A.}$)[mas/yr]&-1.95&-1.94&-1.95&-1.89&-1.96&-2.06&-1.71&-1.71&-1.79&-1.66&-2.24&-2.07&-2.23&-2.17&-2.40&-2.41\\
med(P.M.$_{Dec.}$)[mas/yr]&-3.68&-3.71&-3.68&-3.53&-3.70&-3.67&-3.69&-3.68&-3.81&-3.61&-3.73&-3.75&-3.73&-3.73&-3.62&-3.73\\
$\sigma$med(P.M.$_{R.A.}$)[mas/yr]&0.03&0.07&0.03&0.04&0.04&0.06&0.05&0.05&0.16&0.12&0.10&0.21&0.12&0.13&0.12&0.13\\
$\sigma$med(P.M.$_{Dec.}$)[mas/yr]&0.03&0.08&0.03&0.06&0.03&0.05&0.05&0.05&0.14&0.09&0.07&0.05&0.16&0.18&0.23&0.16\\
f$_{RV}$&0.28&0.07&0.34&0.23&0.36&0.42&0.42&0.38&0.46&0.48&0.29&0.37&0.38&0.47&0.11&0.17\\
med(RV)[km/s]&20.30&19.11&20.30&19.67&20.42&18.71&21.59&21.56&22.25&21.49&20.40&19.18&20.45&20.41&21.85&21.17\\
$\sigma$med(RV)[km/s]&0.39&1.78&0.40&0.46&0.45&0.84&0.68&0.59&0.53&1.98&0.80&0.51&1.80&1.95&0.67&0.61\\


==> xmm19_tab.tex <==
                   n&                R.A.&                Dec.&            id. rad.&              signif&                Cnts&         {Flux (0.3-7.9\,keV)}\\
                    &             [J2000]&             [J2000]&            [arcsec]&                    &                    &    {[10$^{-7}$ph/sec/cm$^2$]}\\
\hline
         1& 06:38:24.65& +10:05:48.5&       6.3&       4.9&      41.5&        51\pm14\\
         2& 06:38:26.30& +10:06:17.9&       6.1&       6.1&      47.7&        56\pm14\\
         3& 06:38:27.77& +09:45:50.0&       2.8&       9.0&      48.2&        34\pm7\\
         4& 06:38:31.49& +09:42:43.7&       4.7&      11.7&     139.6&        66\pm10\\
         5& 06:38:32.83& +09:47:53.3&       6.7&       8.0&     143.3&        51\pm8\\
         6& 06:38:33.05& +09:40:53.1&       3.5&      20.2&     329.3&       103\pm9\\
         7& 06:38:33.46& +09:42:33.6&       2.8&      15.0&     194.3&        58\pm6\\
         8& 06:38:33.65& +10:03:08.9&       8.0&       5.7&      79.5&        42\pm9\\
         9& 06:38:36.77& +10:11:03.7&       3.7&      17.7&     258.5&       119\pm12\\
        10& 06:38:37.23& +09:52:59.3&       6.0&      10.5&     204.7&        73\pm9\\

